HumanNeRF-SE: A Simple yet Effective Approach to Animate HumanNeRF with Diverse Poses

We present HumanNeRF-SE, a simple yet effective method that synthesizes diverse novel pose images with simple input. Previous HumanNeRF works require a large number of optimizable parameters to fit the human images. Instead, we reload these approaches by combining explicit and implicit human representations to design both generalized rigid deformation and specific non-rigid deformation. Our key insight is that explicit shape can reduce the sampling points used to fit implicit representation, and frozen blending weights from SMPL constructing a generalized rigid deformation can effectively avoid overfitting and improve pose generalization performance. Our architecture involving both explicit and implicit representation is simple yet effective. Experiments demonstrate our model can synthesize images under arbitrary poses with few-shot input and increase the speed of synthesizing images by 15 times through a reduction in computational complexity without using any existing acceleration modules. Compared to the state-of-the-art HumanNeRF studies, HumanNeRF-SE achieves better performance with fewer learnable parameters and less training time.

==> sec/4_experiments_1.tex <==
\section{Experiments}

% oldversion
% Our goal is to improve the pose generalization of the methods, so our experiments mainly focus on image synthesis of novel poses rather than synthesizing images from new viewpoints.
% oldversion
% In this section, we conducted experiments on the publicly available dataset \textsc{zju-mocap} and compared it with other state-of-the-art neural radiance field methods that only use SMPL information as prior knowledge for humans. 
% The experiments mainly consisted of two parts: classic novel pose experiments which simply spilt videos to 2 parts in a certain proportion and unseen pose experiments which require that the test poses and training poses are very different to prevent pose leakage issues as much as possible.

\paragraph{Evaluation metrics.}
% For novel view image synthesis, 
% We evaluate our method using 
We use three metrics:  peak signal-to-noise ratio (PSNR),  structural similarity index (SSIM), and learned perceptual image patch similarity (LPIPS). 
It should be noted that LPIPS is the most human-perceptually-aligned metric among these indicators, while PSNR prefers smooth results but may have bad visual quality~\cite{zhang2018unreasonable}.

\paragraph{Dataset.}
We use \textsc{zju-mocap} and our self-captured videos (real-world applicable data) to evaluate our method. We follow~\cite{weng2022humanNeRF}[monohuman]  to select the same 6 subjects in \textsc{zju-mocap} for our evaluation.  
\textsc{zju-mocap} is a dataset that captures the target human body from 23 different perspectives synchronously, We only use the first view captured in each subject.

The previous work did not consider the issue of pose leakage caused by the strong repetition of actions in \textsc{zju-mocap}. In order to further validate the performance of the model, we shot videos using handheld devices. We limited the training videos to a person spinning with A pose, and used diverse action videos for evaluation, which is a more real-world applicable evaluation method.

\paragraph{Compared Methods.}
We compared our method in terms of the performance of image synthesis with the most influential method HumanNeRF~\cite{weng2022humanNeRF} and the latest state-of-the-art method MonoHuman~\cite{yu2023monohuman} which improves the pose generalization of HumanNeRF and works better than~\cite{jiang2022neuman,peng2021neural}. We also take Ani-NeRF~\cite{peng2021animatable} as one of the baselines because this work presents SMPL-based neural blend weight that can better generalize novel poses.


% \todo{The subsection of few-shot should be in the behind of section of Novel pose.}

\begin{table*}[!t]
\centering
\caption{\textbf{Average results of six subjects on \textsc{zju-mocap}}. Our method (green) exhibits excellent quantitative metrics, especially in terms of LPIPS. This indicates that the results of our method are more in line with human visual perception. Our method also achieves faster training and rendering speeds due to our simple and effective architecture.
$^\dagger$LPIPS = 1,000$\times$LPIPS. 
}
\label{tab:fewshot-zjumocap}
\setlength{\tabcolsep}{8pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{lllllllll}
\toprule
& \multicolumn{3}{c}{\textbf{Full}} 
& \multicolumn{3}{c}{\textbf{Few-shot}} & \multicolumn{2}{c}{\textbf{Time}} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
\cmidrule(lr){8-9}

 & \multicolumn{1}{c}{\small{PSNR$\uparrow$}} & \multicolumn{1}{c}{\small{SSIM$\uparrow$}} & \multicolumn{1}{c}{\small{$^\dagger$LPIPS$\downarrow$}} & \multicolumn{1}{c}{\small{PSNR$\uparrow$}} & \multicolumn{1}{c}{\small{SSIM$\uparrow$}} & \multicolumn{1}{c}{\small{$^\dagger$LPIPS$\downarrow$}} 
 & \multicolumn{1}{c}{\small{Train}}
 & \multicolumn{1}{c}{\small{Render}}
 \\ 
\midrule     
% & PSNR & SSIM & LPIPS*   \\ \hline
Ani-NeRF~\cite{peng2021animatable} &21.24989 & 0.845823 & 68.221 &22.18072 & 0.833925 & 64.839 & ~40h &2.73s/it \\

HumanNeRF~\cite{weng2022humanNeRF} & {31.15863} \gold & 0.973859 & 24.822 & 29.90272 & 0.968346 & 33.056 & ~56h & 2.37s/it\\

MonoHuman~\cite{yu2023monohuman} & 30.90996 & 0.971814 & 31.292 & 30.10187& 0.967719  & 36.494 & ~70h & 5.96s/it\\

\rowcolor{CBLightGreen} Ours  & 31.09413 & {0.974030} \gold & {24.085} \gold & {30.11349} \gold & {0.968382} \gold  & {32.084} \gold  & 2.5h \gold &0.16s/it \gold \\

\midrule
HumanNeRF~\cite{weng2022humanNeRF}  &28.97  &0.962901 &48.128 & & & & &  \\
MonoHuman~\cite{yu2023monohuman} &29.15 &0.963873 &51.623 & & & & & \\
Ours &29.23 &0.966557 &46.308 & & & & & \\
 
\bottomrule
\end{tabular}
}

\end{table*}

\begin{table}[]
\centering
\label{tab:custom}
\caption{\textbf{Average results of real-world applicable data.} Our method demonstrates comprehensive advantages on real-world applicable data. \todo{TODO: merge it with table 1(merge problem--Time)}}
\begin{tabular}{llll}
\toprule
          & \multicolumn{1}{c}{PSNR$\uparrow$} & \multicolumn{1}{c}{SSIM$\uparrow$} & \multicolumn{1}{c}{$^\dagger$LPIPS$\downarrow$} \\
          \midrule
HumanNeRF & 28.97  & 0.9629   & 48.128  \\
MonoHuman & 29.15  & 0.9638   & 51.623  \\
Ours      & 29.23 \gold  & 0.9666 \gold   & 46.308 \gold  \\ 
\bottomrule
\end{tabular}
\end{table}

\todo{Do not use novel pose and few shot as two sections. Use qualitative evaluation and quantitative evaluation.}

\subsection{Novel Pose}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{images/novelpose6.png}
    \caption{The synthesis result of novel pose. For \textsc{zju-mocap}, we used the pose of Subject 387 to drive other performers to generate novel poses. For these performers, the synthesized poses are not trained during the training process.  
    % The results of HumanNeRF~\cite{weng2022humanNeRF} appeared with artifacts and unrealistic distortions in many places, while we synthesized the images of the performers more realistically.
    For in-the-wild data, we trained our model using videos of performers simply rotating and synthesized novel poses in completely different videos of the same performer.
    }
    \label{fig:novelpose}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.9\textwidth]{images/fewshot5.pdf}
    \caption{\textbf{Results with fewshot training images.} Because of limited information used in training, previous methods~\cite{weng2022humanNeRF,yu2023monohuman} were unable to learn appropriate human weights. HumanNeRF~\cite{weng2022humanNeRF} exhibits distortion and artifacts. The performance of Monohuman~\cite{yu2023monohuman} is even worse because it is difficult to find suitable reference images. Our method maintains stability in image structure under few-shot data input.}
    \label{fig:fewshot}
\end{figure*}


In previous work, the experiments of novel pose were usually trained with the first half of a video and evaluated with the remaining half. 
We considered this kind of evaluation limited because the poses used for evaluation were highly similar to those used for training in the most used \textsc{zju-mocap}. 

A simple way to avoid pose leakage problem is to use completely different action sequences as evaluation. 
But as there is no ground truth of \textsc{zju-mocap}, we provided comparison results as Figure~\ref{fig:novelpose}, and synthesized over 200 zero-shot pose images and converted them into 20 videos, which were subjectively evaluated by six or more evaluators as shown in Figure~\ref{fig:subjective-reasearch}.


The entire evaluation process is single-blind, meaning that the evaluators do not know which specific method generated the results. We also included some test seeds, which serve as the Ground Truth, and all of these seeds received high scores from the evaluators, indicating that their evaluations were professional and objective. The evaluators were asked to evaluate the video in terms of image distortion, artifacts, details, plausibility, and precision, and to provide a final score that was assigned to one of three different levels.

As a result, almost all the evaluators subjectively think our results have a better performance. Our results were classified as perfect in significantly higher numbers than HumanNeRF, with fewer votes for flaws. However, both the results performed poorly in cases of poor data quality.

To quantitatively compare the results of the novel pose and make the data more applicable to real-world scenarios, we captured data in the living room and wild.



\begin{figure}
  \centering
  \begin{subfigure}[b]{0.4\linewidth}
    \includegraphics[width=\linewidth]{images/humanNeRF-subject.png}
    \caption{HumanNeRF\cite{weng2022humanNeRF}}
    \label{fig:humanNeRF-sub}
  \end{subfigure}
  \quad
  \begin{subfigure}[b]{0.4\linewidth}
    \includegraphics[width=\linewidth]{images/ours-subject.png}
    \caption{Ours}
    \label{fig:ours-sub}
  \end{subfigure}
  \caption{\textbf{Subjective evaluation results.} We use cross-rendering of different subjects in the \textsc{zju-mocap} to ensure that the evaluation of the novel pose is sufficiently novel. Our results were evaluated to have a significantly higher perfect proportion than HumaneNeRF.}
  \label{fig:subjective-reasearch}
\end{figure}

% \begin{table}[t]
% \centering
% \caption{Subjective image evaluation results, \todo{Change to figure}}
% \begin{tabular}{c|l|l|l|l}
% %\hline
%  & perfect & flawed & Problematic & Average \\ 
% \midrule[1.5pt]
%  HumanNeRF~\cite{weng2022humanNeRF} & 13 & 87 & 22 & 5.8 \\ \hline
%  Ours & 49 & 49 & 22 & 6.7 
% \end{tabular}
% \label{table:subjectiveresults}
% \end{table}


The results showed that when the target pose differed significantly from the training data, HumanNeRF~\cite{weng2022humanNeRF} produced noticeable artifacts, which greatly decrease the image quality, while our method still produced highly realistic results for zero-shot pose synthesis. We believe that there are two reasons for this. First, HumanNeRF's neural weight field relies on the diversity of the training data and thus does not perform well on zero-shot pose synthesis, while our approach is based on SMPL vertex weights, which have good pose generalization ability. Second, HumanNeRF utilizes frame-level features to reduce SMPL noise and optimize results during training, while we only use point-level features to improve novel view metrics, making our method less likely to overfit.



\subsection{Few-shot Performance}
% 



The previous method has overfitting problems in synthesizing novel poses, which is more obvious when the input is limited.
To further conduct quantitative experiments on public dataset \textsc{zju-mocap}, we refer to the previous experiment settings.
For any set of data in \textsc{zju-mocap}, we divided the data into training and testing data in a 4:1 ratio, which follows the setting of previous work. Differently, we uniformly select only about 30 frames from the divided training part as few-shot input. This setting can effectively avoid pose leakage compared to the full input
Our experimental results in \textsc{zju-mocap} with few-shot training images are shown in Table~\ref{tab:fewshot-zjumocap}. 





% 

% \begin{table*}[!t]
% \begin{tabular}{clll}
% & \multicolumn{3}{c}{Full} \\
%  & \multicolumn{1}{c}{\small{PSNR$\uparrow$}} & \multicolumn{1}{c}{\small{SSIM$\uparrow$}} & \multicolumn{1}{c}{LPIPS*$\downarrow$} \\ 
% \midrule[1.5pt]          
% % & PSNR & SSIM & LPIPS*   \\ \hline
% HumanNeRF & {31.15863} \gold & 0.973859 & 24.822 \\
% MonoHuman & 30.90996 & 0.971814 & 31.292 \\
% Ours  & 31.09413 & {0.974030} \gold & {24.085} \gold \\
% \end{tabular}
% \begin{tabular}{clll}
% & \multicolumn{3}{c}{Few-shot} \\

% & \multicolumn{1}{c}{\small{PSNR$\uparrow$}} & \multicolumn{1}{c}{\small{SSIM$\uparrow$}} & \multicolumn{1}{c}{LPIPS*$\downarrow$} \\ 
% \midrule[1.5pt]
% HumanNeRF & 29.90272 & 0.968346 & 33.056 \\
% MonoHuman & 30.10187& 0.967719  & 36.494 \\
% Ours      & {30.11349} \gold & {0.968382} \gold  & {32.084} \gold
% \end{tabular}
% \caption{ \textbf{Average results of six subjects on \textsc{zju-mocap}}, }
% \label{tab:fewshot-zjumocap}
% \end{table*}



==> sec/intro_backup.tex <==
\section{Introduction}
\label{sec:intro}




\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/motivation15.pdf}
    \vspace{-3mm}
    \caption{
    \textbf{Different weights for deformation.} 
    (a) Prior methods~\cite{peng2021animatable,weng2022humannerf,yu2023monohuman,liu2021neural} learn weight volume through neural networks or fine-tune SMPL weight. When synthesizing novel pose images, points tend to be deformed onto the canonical space \emph{incorrectly} because of the over-fitted weight, leading to artifacts.
    (b) Simply using the nearest SMPL vertex's LBS (Linear Blending Skinning) weight
    % through methods such as KNN. 
    % This method 
    leads to the sampling space being filled with colors related to the clothes, which we named %it 
    color bleeding. For the given data, the performer's regular punching causes many transparent points %are 
    to be deformed onto the T-shirt in the canonical space, leading to convergence in the color bleeding space. For leg movements pose, points in the space also deform onto the other leg in the canonical space.
    (c) We perform convolution filtering in the voxel volume and then query the nearest SMPL vertex's LBS weight. This architecture is simple yet effective. Our method not only avoids overfitting but also greatly reduces the required size of the neural network and achieves performance improvement.
    }
    \vspace{-5mm}
    \label{fig:motivation}
\end{figure}



% \begin{table}[h]
%     \centering
%     \begin{tabular}{l|l}
%     \hline
%      & animatable \\ \hline
%     UV calculation   & \cite{liu2021neural,peng2023intrinsicngp,chen2023uv,geng2023learning} \\ \hline
%     without UV   & \cite{peng2021neural,peng2021animatable,weng2022humannerf,jiang2023instantavatar},ours \\ \hline
%     without SMPL  & \cite{jayasundara2023flexnerf}  
%     \\ \hline
%     \end{tabular}
%     \caption{Categorization of human NeRF methods.}
%     \label{tab:Categorization}
% \end{table}
The prevalence of human-centric videos recorded on handheld devices has led to a growing need for technologies capable of analyzing, reconstructing, and synthesizing photo-realistic human appearances from monocular video sequences. This need is critical for various gesture-controlled applications such as human-computer interactions and gaming. 

However, achieving this goal is challenging due to the limited and patchy representations of human bodies typically present in monocular videos.
Although there are methods~\cite{jiang2022neuman,weng2022humannerf,yu2023monohuman,jiang2023instantavatar,geng2023learning} % cite some papers here
that can learn high-quality human representations from monocular videos and synthesize images from arbitrary viewpoints, they cannot perform well in synthesizing \emph{novel pose} images that are significantly \emph{different} from the training videos and they usually take long time to train. These limitations restrict the potential application scenarios of these techniques. 

% A particularly challenging aspect of this task is extracting human representations from a limited number of monocular videos and generating images of the human body in arbitrary zero-shot poses. The learned pose from limited monocular videos is often simple and cannot cover all human poses, requiring methods to learn human representation from simple poses and synthesize human images entirely different from the training data.

To address this limitation, a crucial challenge is to generate human body images in arbitrary zero-shot poses from monocular videos with limited poses.
This task is exceptionally challenging. Unlike multi-camera videos that contain more informative data, limited poses provided by monocular videos are often simplistic and cannot encompass all possible human body poses. 
We need to employ methods to learn implicit human representations from simple poses and synthesize human body images that are entirely different from the training data. Simultaneously, it is crucial to minimize training time and enhance the efficiency of the methods as much as possible, making it more practical for applications.


% The NeRF-based approach~\cite{mildenhall2021nerf} has demonstrated strong potential to address the problem, whereby a set of implicit neural representations are learned directly from images. Through differentiable rendering, the 3D spatial samples are aggregated to fit the recorded RGB observations. 
% The key challenge lies in mapping the observed space sampling points to a canonical space. 
% Previous methods have introduced priors on body pose and shape, and normalized the representation and sampling strategies of the samples from the scene through various techniques to learn the latent representation of the human body. NeuralBody~\cite{peng2021neural} learns the implicit human body representation by encoding a dense SMPL~\cite{loper2015smpl} grid, where the sample points are anchored to the grid vertices. AnimatableNeRF~\cite{peng2021animatable} and HumanNeRF~\cite{weng2022humannerf} warp the observed space sampling points to the T-pose space by learning a mixture of neural weights. NeuralActor~\cite{liu2021neural} and some methods~\cite{peng2023intrinsicngp,geng2023learning} further anchor the sampling points with respect to the body UV representation. 


% methods such as
Previous works ~\cite{wu2020multi,habermann2020deepcap,xu2018monoperfcap,liu2019neural,saito2020pifuhd,xiu2022icon} typically employ point clouds and textured meshes to optimize a tailless three-dimensional structure, which need to be translated into images, limiting their applicability. 

Differently, neural rendering-based methods~\cite{wang2021ibrnet,zhang2020nerf++,niemeyer2021giraffe,wu2022dof,wang2022nerf} can directly achieve satisfactory image synthesis results.
However, they typically assume multi-camera inputs and do not account for object deformation. 
Deformable methods~\cite{park2021nerfies,park2021hypernerf,pumarola2021d,tretschk2021non,xian2021space}  extend upon this by endowing implicit fields with the capability to express dynamic objects. 
Nevertheless, these methods perform poorly on humans, due to the complex deformation of motions.

% Subsequent research aims to address the issue of human body deformation. 
To address the issue of human body deformation, some studies~\cite{kwon2021neural,peng2021animatable,peng2021neural,liu2021neural,zhao2022humannerf,chen2023uv}  leverage NeRF to learn dynamic human representations from multi-camera images and some of them can generalize to novel poses. 
However, the increasing data and equipment requirements 
% associated with multi-camera data, including hardware, camera alignment, and storage, 
limited their practical applicability. 
Certain monocular methods~\cite{jiang2022neuman,weng2022humannerf,yu2023monohuman,jiang2023instantavatar,geng2023learning} eased data constraints by allowing the utilization of monocular videos as input. 
HumanNeRF~\cite{weng2022humannerf} showcases remarkable novel view results by decoupling the motion field. It utilizes extensive neural networks to fit various modules, often requiring a considerable amount of time for training. MonoHuman~\cite{yu2023monohuman} further improves the capability to synthesize novel pose images by using reference images and bidirectional constraints. This results in longer time requirements and poor results when there is a large difference between the training poses and the rendering poses.
Moreover, when the input poses become more limited, the aforementioned methods often yield highly unsatisfactory results due to overfitting of their neural weight (Figure~\ref{fig:motivation}).


% Among them, NeuralActor has achieved excellent results in driving the human body, but the demand for texture relative to other readily attainable SMPL limits its usefulness.

We present HumanNeRF-SE, which can synthesize novel pose images with tens of simple inputs and a few learnable parameters in hours. 
Our approach distinguishes itself from previous methods by effectively preventing potential overfitting while maintaining a robust correlation between human NeRF representation and prior pose.
Furthermore, our technique does not depend on a diverse range of motion samples to improve generalization performance under varying poses. 
% Instead, we take advantage of the publicly accessible SMPL model to enable generalization to any zero-shot pose.
To begin, we want to extract the relation between explicit SMPL vertices and sampling points. 
To achieve this, we convert the SMPL vertex coordinates into a voxelized form and employ an adaptive unified kernel to diffuse the vertices across the voxel volume. 
Following this, the spatial-aware feature and occupancy of the sampling point can be easily queried in this volume, and contribution comes from all vertices within the receptive field centered on the sampling point. 
Throughout this procedure, a significant number of points unrelated to the body are filtered out, leaving behind only those points likely to be related to the human body. These points can be deformed to a unified canonical pose to get the coarse coordinates. 
We refine the coarse coordinates by performing a specific mapping using the point-level spatial-aware feature obtained in the convoluted voxel volume.
Finally, we get the colors and densities of the sampling points through a neural network and render the image through a differentiable renderer.

Overall, we propose a novel HumanNeRF method that can synthesize images of varying poses simply yet effectively. 
Our approach utilizes explicit SMPL vertices and leverages a general and specific mapping process to model the deformation from observation to canonical space. 
Our experiments show that our method can generate novel poses with significant differences from the training poses, even when the input is limited to a few shots.
To further demonstrate the performance of our method, we captured in-the-wild data, where the input video involves a simple rotation of the user.

In summary, this work makes the following contributions:
\begin{itemize}
    \item We use an adaptive space conv-filter and frozen deformation weights for the general mapping process. This greatly reduces computational complexity and avoids overfitting.
    \item We design a spatial-aware feature point refine module as our specific mapping process to reduce the unnatural sharp results caused by rigid deformation.
    \item Our architecture is simple yet effective. Compared to methods with similar performance, HumanNeRF-SE uses less than 1\% learnable parameters, 1/20 training time, and increases rendering speed by 15 times without using any existing acceleration modules.
\end{itemize}




==> sec/table_used.tex <==
% 分subject的fewshot table
\begin{table*}[]
\centering
\begin{minipage}{\textwidth}
\centering
\begin{tabular}{llllllllll}
& \multicolumn{3}{c|}{Subject377}    & \multicolumn{3}{c|}{Subject386}    & \multicolumn{3}{c}{Subject387}\\ 
% \midrule
& \small{\small{PSNR$\uparrow$}} & \small{SSIM$\uparrow$}  & \small{LPIPS$\downarrow$}   & \small{PSNR$\uparrow$} & \small{SSIM$\uparrow$}  & \small{LPIPS$\downarrow$}   & \small{PSNR$\uparrow$} & \small{SSIM$\uparrow$}  & \small{LPIPS$\downarrow$} \\ \midrule
MonoHuman & 31.02 & 0.9774 & 22.56 & 31.26 & 0.9601 & 56.92 & {28.50} \gold  & {0.9619} \gold & 43.15  \\
HumanNeRF & 30.33 & 0.9799 & 18.51 & 31.47 & 0.9618 & 48.41 & 27.92 & 0.9610  & 39.94                         \\
Ours  & {31.07} \gold & {0.9806} \gold & {18.48} \gold & {32.44} \gold & {0.9644} \gold & {43.87} \gold & 28.05 & 0.9612 & {39.73} \gold\\
\end{tabular}
\end{minipage}
\rule{0pt}{1ex}
\begin{minipage}{\textwidth}
\centering
\begin{tabular}{l|lll|lll|lll}
& \multicolumn{3}{c|}{Subject392}    & \multicolumn{3}{c|}{Subject393}    & \multicolumn{3}{c}{Subject394}  \\ \midrule
& \small{PSNR$\uparrow$} & \small{SSIM$\uparrow$}  & \small{LPIPS$\downarrow$}   & \small{PSNR$\uparrow$} & \small{SSIM$\uparrow$}  & \small{LPIPS$\downarrow$}   & \small{PSNR$\uparrow$} & \small{SSIM$\uparrow$}  & \small{LPIPS$\downarrow$}\\ \midrule
MonoHuman & 31.48 & 0.9739 & 30.09 & 29.45 & 0.9691 & 30.11 & {28.86} \gold & {0.9636} \gold & 36.14 \\
HumanNeRF & {31.55} \gold & {0.9747} \gold & 28.04 & {29.45} \gold & {0.9694} \gold & {26.93} \gold & 28.66 & 0.9629 & 36.51  \\
Ours  & 31.36 & 0.9734 & {27.60} \gold & 29.25 & 0.9681 & 27.32 & 28.51 & 0.9626 & {35.47} \gold
\end{tabular}
\end{minipage}
\caption{Comparison of few-shot training images results on the \textsc{zju-mocap} dataset. }
\label{tab:fewshot-zjumocap}
\end{table*}



% pose simi table
\begin{table}[]
\begin{tabular}{cccc}
    & Min   & Max   & Average     \\ \hline
377 & 0.876 & 0.997 & 0.919       \\
386 & 0.939 & 0.995 & 0.964       \\
387 & 0.969 & 0.996 & 0.985       \\
392 & 0.845 & 0.957 & 0.909       \\
393 & 0.834 & 0.998 & 0.904       \\
394 & 0.760 & 0.993 & 0.842      
\end{tabular}
\caption{Pose similarity of test poses and train poses in previous novel pose experiments. The setting is not novel enough because of the high similarity. \todo{move to supp}}
\label{tab:posesimi}
\end{table}


% monocular methods 的对比
\begin{table}[]
\begin{tabular}{lll}
Name  & Animatable & w/o UV/Mesh   \\ \hline
AniNeRF~\cite{peng2021animatable} & \checkmark &        \\

NeuMan~\cite{jiang2022neuman} & \checkmark    &    \\
InstantAvatar~\cite{jiang2023instantavatar} & \checkmark       &  \checkmark  \\
IntrinsicNGP~\cite{peng2023intrinsicngp}  &           &  \\
InstantNVR~\cite{geng2023learning}   &     &       \\ 
HumanNeRF~\cite{weng2022humannerf}
& \checkmark    & \checkmark  \\
Monohuman~\cite{yu2023monohuman}     & \checkmark    &  \checkmark     \\
\hline
Ours  & \checkmark    &\checkmark  
\end{tabular}
\caption{NeRF based human images synthesis methods with monocular data. We selected the most similar and latest method and the most influential method as our baselines.}
\label{tab:methodscompare}
\end{table}
